Multi-View Spectral Clustering Tailored Tensor Low-Rank Representation

This paper explores the problem of multi-view spectral clustering (MVSC) based on tensor low-rank modeling. Unlike the existing methods that all adopt an off-the-shelf tensor low-rank norm without considering the special characteristics of the tensor in MVSC, we design a novel structured tensor low-rank norm tailored to MVSC. Specifically, we explicitly impose a symmetric low-rank constraint and a structured sparse low-rank constraint on the frontal and horizontal slices of the tensor to characterize the intra-view and inter-view relationships, respectively. Moreover, the two constraints could be jointly optimized to achieve mutual refinement. On the basis of the novel tensor low-rank norm, we formulate MVSC as a convex low-rank tensor recovery problem, which is then efficiently solved with an augmented Lagrange multiplier based method iteratively. Extensive experimental results on five benchmark datasets show that the proposed method outperforms state-of-the-art methods to a significant extent. Impressively, our method is able to produce perfect clustering. In addition, the parameters of our method can be easily tuned, and the proposed model is robust to different datasets, demonstrating its potential in practice.

==> figures.tex <==
\begin{figure}[!t]
	\begin{minipage}[b]{0.325\linewidth}
		\centering
		\centerline{\epsfig{figure=orl-visual-LTMSC-c-v2,width=2.8cm}}
		%		\vspace{-0.1cm}
		\centerline{ORL: LT-MSC}\medskip
	\end{minipage}
	\begin{minipage}[b]{0.325\linewidth}
		\centering
		\centerline{\epsfig{figure=orl-visual-jet-ijcv-h-c,width=2.8cm}}
		%		\vspace{-0.1cm}
		\centerline{ORL: t-SVD-MSC}\medskip
	\end{minipage}
	\begin{minipage}[b]{0.325\linewidth}
		\centering
		\centerline{\epsfig{figure=orl-visual-jet-proposed-h-c,width=2.8cm}}
		%		\vspace{-0.1cm}
		\centerline{ORL: Proposed}\medskip
	\end{minipage}\\
	\begin{minipage}[b]{0.325\linewidth}
		\centering
		\centerline{\epsfig{figure=yaleB-visual-LTMSC-c,width=2.8cm}}
		%		\vspace{-0.1cm}
		\centerline{YaleB: LT-MSC}\medskip
	\end{minipage}
	\begin{minipage}[b]{0.325\linewidth}
		\centering
		\centerline{\epsfig{figure=yaleB-visual-jet-ijcv-h-c,width=2.8cm}}
		%		\vspace{-0.1cm}
		\centerline{YaleB: t-SVD-MSC}\medskip
	\end{minipage}
	\begin{minipage}[b]{0.325\linewidth}
		\centering
		\centerline{\epsfig{figure=yaleB-visual-jet-proposed-h-c,width=2.8cm}}
		%		\vspace{-0.1cm}
		\centerline{YaleB: Proposed}\medskip
	\end{minipage}
	\caption{Visual comparisons  of the similarity matrices constructed by different methods. Due to the space limitation, only the results of three low-rank tensor based methods are shown on two datasets. It is clear that the connections of our method distribute along the diagonal,  
	and our method generates much fewer wrong connections than the compared methods.}
	\label{fig:visual}
\end{figure}

\begin{figure}[!t]
	\begin{minipage}[b]{0.325\linewidth}
		\centering
		%		\centerline{\epsfig{figure=para_w1_v4.eps,width=4.2cm}}
		\centerline{\epsfig{figure=para_orl_w1.eps,width=3.2cm}}
		%		\vspace{-0.1cm}
		%%		\centerline{(a) YaleB: IJCV}\medskip
	\end{minipage}
	\begin{minipage}[b]{0.325\linewidth}
		\centering
		%		\centerline{\epsfig{figure=para_alpha.eps,width=4.2cm}}
		\centerline{\epsfig{figure=para_orl_alpha.eps,width=3.2cm}}
		%		\vspace{-0.1cm}
		%		\centerline{(a) YaleB: IJCV}\medskip
	\end{minipage}
	\begin{minipage}[b]{0.325\linewidth}
		\centering
		%		\centerline{\epsfig{figure=para_lambda.eps,width=4.2cm}}
		\centerline{\epsfig{figure=para_orl_lambda.eps,width=3.2cm}}
		%		\vspace{-0.1cm}
		%		\centerline{(a) YaleB: IJCV}\medskip
	\end{minipage}\\
	\begin{minipage}[b]{0.325\linewidth}
		\centering
		\centerline{\epsfig{figure=para_coil20_w1,width=3.2cm}}
		%		\vspace{-0.1cm}
		%		\centerline{(a) YaleB: IJCV}\medskip
	\end{minipage}
	\begin{minipage}[b]{0.325\linewidth}
		\centering
		\centerline{\epsfig{figure=para_coil20_alpha,width=3.2cm}}
		%		\vspace{-0.1cm}
		%		\centerline{(a) YaleB: IJCV}\medskip
	\end{minipage}
	\begin{minipage}[b]{0.325\linewidth}
		\centering
		\centerline{\epsfig{figure=para_coil20_lambda,width=3.2cm}}
		%		\vspace{-0.1cm}
		%		\centerline{(a) YaleB: IJCV}\medskip
	\end{minipage}
	\caption{Illustration of the effect of three hyper-parameters of our model (i.e., $\omega_1,\lambda$ and $\alpha$) on the clustering performance. It can be observed that the proposed method always achieves the highest performance in large ranges of $\omega_1,\lambda$ and $\alpha$, demonstrating its robustness.}
	\label{fig:para}
\end{figure}
